FPGA Synthesis of Ternary Memristor-CMOS Decoders

The search for a compatible application of memristor-CMOS logic gates has remained elusive, as the data density benefits are offset by slow switching speeds and resistive dissipation. Active microdisplays typically prioritize pixel density (and therefore resolution) over that of speed, where the most widely used refresh rates fall between 25-240 Hz. Therefore, memristor-CMOS logic is a promising fit for peripheral IO logic in active matrix displays. In this paper, we design and implement a ternary 1-3 line decoder and a ternary 2-9 line decoder which are used to program a seven segment LED display. SPICE simulations are conducted in a 50-nm process, and the decoders are synthesized on an Altera Cyclone IV field-programmable gate array (FPGA) development board which implements a ternary memristor model designed in Quartus II. We compare our hardware results to a binary coded decimal (BCD)-to-seven segment display decoder, and show our memristor-CMOS approach reduces the total IO power consumption by a factor of approximately 6 times at a maximum synthesizable frequency of 293.77MHz. Although the speed is approximately half of the native built-in BCD-to-seven decoder, the comparatively slow refresh rates of typical microdisplays indicate this to be a tolerable trade-off, which promotes data density over speed.

==> tables.tex <==
% \begin{table}[!t]\scriptsize
% \centering\caption{Positive Ternary Logic Gate Truth Table}
% \begin{tabular}{
% >{\columncolor[HTML]{FFFFFF}}l 
% >{\columncolor[HTML]{FFFFFF}}l
% >{\columncolor[HTML]{FFFFFF}}l
% >{\columncolor[HTML]{FFFFFF}}l}
% \hline\vspace{-6pt}
%  &   \\ \hline
 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{v$_{\rm in1}$}} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{v$_{\rm in2}$}} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{TAND}}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{TOR}}\\ \hline

% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} \\ \hline

% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} \\ \hline

% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} \\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} \\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} \\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} \\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} \\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}\\ \hline


% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} \\ \hline

 
% \hline \vspace{-6pt}
%   &  \\ \hline
% \end{tabular}%
% \end{table}



% \begin{table}[!t]\scriptsize
% \centering\caption{Unbalanced TI Truth Table}
% \begin{tabular}{
% >{\columncolor[HTML]{FFFFFF}}l 
% >{\columncolor[HTML]{FFFFFF}}l
% >{\columncolor[HTML]{FFFFFF}}l
% >{\columncolor[HTML]{FFFFFF}}l}
% \hline\vspace{-6pt}
% &   \\ \hline
% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{v$_{\rm in}$}} & 
% \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{STI}} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{PTI}} 
% & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{NTI}} \\ \hline

% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}0} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} &
% \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2}  \\ 
 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}1} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1} &
% \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}0}  \\ 
 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}2} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} &
% \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}0} &  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}0}  \\ 
 
% \hline \vspace{-6pt}
%  &  \\ \hline
% \end{tabular}%
% \end{table}



\begin{table}[!t]\scriptsize
\centering\caption{Ternary Display Decoder Truth Table}
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l}
\hline\vspace{-6pt}
 &   \\ \hline
 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$A$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline


\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$B$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_a$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_b$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_c$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_d$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_e$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_f$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{$Y_g$}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}\\ \hline

\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}Display}} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}
& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0}\\ \hline

\hline \vspace{-6pt}
  &  \\ \hline
\end{tabular}%
\end{table}
